Sister Help: Data Augmentation for Frame-Semantic Role Labeling

While FrameNet is widely regarded as a rich resource of semantics in natural language processing, a major criticism concerns its lack of coverage and the relative paucity of its labeled data compared to other commonly used lexical resources such as PropBank and VerbNet. This paper reports on a pilot study to address these gaps. We propose a data augmentation approach, which uses existing frame-specific annotation to automatically annotate other lexical units of the same frame which are unannotated. Our rule-based approach defines the notion of a sister lexical unit and generates frame-specific augmented data for training. We present experiments on frame-semantic role labeling which demonstrate the importance of this data augmentation: we obtain a large improvement to prior results on frame identification and argument identification for FrameNet, utilizing both full-text and lexicographic annotations under FrameNet. Our findings on data augmentation highlight the value of automatic resource creation for improved models in frame-semantic parsing.

==> 0-abstract.tex <==
\begin{abstract}
%Add S about SRL and FN.
% \swabha{Removed the footnote here because it's hard to have the same footnote in other formats outside of the paper pdf where the abstract needs to be submitted...}
% \swabha{Removing citations from the abstract as well...}
% We tested a hypothesis about the use of existing frame-specific annotation to provide annotation for lexical units (LUs)\footnote{LUs are the unit of analysis in FN. See \ref{LU}.} of the same frame where none exists. 

While FrameNet is widely regarded as a rich resource of semantics in natural language processing, a major criticism concerns its lack of coverage and the relative paucity of its labeled data compared to other commonly used lexical resources such as PropBank and VerbNet. This paper reports on a pilot study to address these gaps. We propose a data augmentation approach, which uses existing frame-specific annotation to automatically annotate other lexical units of the same frame which are unannotated. Our rule-based approach defines the notion of a \textbf{sister lexical unit} and generates frame-specific augmented data for training. We present experiments on frame-semantic role labeling which demonstrate the importance of this data augmentation: we obtain a large improvement to prior results on frame identification and argument identification for FrameNet, utilizing both full-text and lexicographic annotations under FrameNet. Our findings on data augmentation highlight the value of automatic resource creation for improved models in frame-semantic parsing.
% https://aircconline.com/csit/abstract/v10n12/csit101201.html
\end{abstract}

==> 1-intro.tex <==
\section{Introduction}
\label{sec:intro}



Among the challenges to Natural Language Processing (NLP) systems is access to sufficient and accurate information about the mapping between form and meaning in language \citep{benderkoller20climbing}. 
While the number of resources that provide such information has increased in recent decades, producing these resources remains labor-intensive and costly.
This is particularly true for FrameNet (\textbf{FN}; \citealp{Ruppenhofer:16}), a rich resource of semantic annotations, popularized for semantic role labeling (\textbf{SRL}) since the pioneering work of \citet{Dans02}.
% Since the pioneering work of \citet{Dans02}, semantic role labeling (\textbf{SRL}) is a mainstay in core NLP, such as event extraction, participant tracking, machine translation, and question-answering, 
% including most recently where \citet{conianavigli20bridg} showed an improvement in results with low-resource languages when adopting a language-agnostic approach to SRL. 

Nevertheless, FrameNet still relies (almost exclusively) on expert manual linguistic annotation, resulting in far fewer annotations than other resources that are able to scale up the annotation process easily \cite{fitzgerald-etal-2018-large}.
Moreover, the fine-grained annotations in FrameNet make them harder to produce compared to other lexical resources such as PropBank \citep{propbank} and VerbNet \citep{verbnet}.
As a result, while SRL has continued to be a mainstay of core NLP, with applications in event extraction, participant tracking, machine translation, and question-answering, far fewer SRL systems use FrameNet for training, in contrast to PropBank.\footnote{PropBank annotations were also included in CoNLL shared tasks in 2005 \cite{carreras-marquez-2005-introduction} and 2012 \cite{pradhan-etal-2012-conll}, and in OntoNotes \cite{pradhan-etal-2013-towards}.}

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{sections/figures/sister-help.pdf}
\caption{Illustration of Sister Lexical Units (\textbf{Sister LUs}) with FrameNet annotation for the verbs \textit{buy} and \textit{purchase}, which are defined in terms of the \texttt{Commerce\_buy} frame.
The arguments of both LUs are identical, both realizing the frame elements (FEs) \textsc{{\textcolor{blue}{Buyer}}}, \textsc{{\textcolor{green}{Goods}}}, \textsc{{\textcolor{red}{Seller}}}, and \textsc{{\textcolor{violet}{Money}}}.
Targets in the sentence that trigger the frame are the words \textit{bought} and \textit{purchased}, respectively.
}
\label{fig:illustration}
\end{figure}


Our work seeks to address this low resource problem in FrameNet in English by automatic data augmentation.
We leverage the FrameNet hierarchy where multiple lexical units are associated with the same frame, but might have a different number of annotations associated with them (\S\ref{sec:background}).
We propose a rule-based approach to transfer annotations among sister LUs; see Fig. \ref{fig:illustration} for an illustration. 
We implement and extend the proposal by 
\citet{FSautoanno19} to generate new annotation for previously unannotated LUs in the same frame, by exploiting the already identified target and frame of a given lemma.
%\footnote{The authors submitted a preliminary proposal to NSF for consideration in its EAGER program.} 
% NI: footnote really necessary???
% outlined an approach to Frame-SRL that seeks to leverage existing annotation in a frame 
%\textbf{NI:} maybe reword: "...outlined an approach to SRL that seeks to leverage existing annotations for LUs associated with a given frame to generate new annotations for previously unannotated LUs in the same frame, by exploiting the already identified target and frame of a given lemma.
% Reference: Hermann et al. 2014 state of art frame ID system.
% This paper presents a basic implementation of this approach as a proof of concept. 
We hypothesize that our rule-based approach to transfer \textit{{frame-specific}} annotation to generate semantic role labels for example sentences of lexical units (\textbf{LU}s) for which none exist, can indeed result in a FrameNet with higher coverage annotations, a state of affairs that 
can help in training frame-semantic role labeling systems (\S\ref{sec:methodology}).
Our experiments show that this is indeed the case; models trained on augmented data are able to surpass a strong baseline (\sesame; \citealp{DBLP:journals/corr/SwayamdiptaTDS17}) for frame and argument identification (\S\ref{sec:experiments}).
We also provide a summary of the types of linguistic errors in the augmented data and the SRL task.


While our work provides a proof of concept, its novelty lies in exploiting frame-specific annotation to produce augmented data yielding new annotation.
Our implementation and augmented data are publicly available.\footnote{\url{https://github.com/ayush-pancholy/sister-help}}

%\textbf{NI:} Replace the bit starting "The present work..." with : Most recently developed SRL software relies on the availability of sizable amounts of annotated data to provide fodder for machine learning; however, potential sources of such annotated data, such as that provided by the FrameNet project, are relatively sparse due to the high cost of manual annotation. To address the need for larger bodies of data, we have explored means to automatically generate reliable semantic role annotations by leveraging existing \textbf{\underline{frame-specific}} annotations in FrameNet. In particular, we explore the potential  to generate annotated example sentences for lexical units already present in FrameNet, but which currently lack associated examples.

%including recently \citet{xiaetal2020srl}, which addressed SRL using heterogeneous syntactic knowledge, and \citet{klein20qanom}, which advanced SRL work of nominal dependents, derived from question-answering.

% The rest of the paper proceeds as follows here: Section \ref{sec:background} provides background information about FrameNet and SRL; Section \ref{sec:related} covers related work; Section \ref{sec:methodology} describes the hypothesis motivating the current effort and the methodology used to generate the augmented data; Section \ref{sec:experiments} presents the experiments and their results, as well as a summary of the types of linguistic errors in the augmented data and the SRL task; and Section \ref{sec:future} looks to future work.

==> 2-background.tex <==
\section{Background}
\label{sec:background}

\subsection{FrameNet}
FrameNet \citep{Ruppenhofer:16} is a research and resource development project in corpus-based computational lexicography grounded in the principles of \textbf{frame semantics} \citep{Fillmore:85}.
One of
the goals of this effort 
is documenting the \textbf{valences}, i.e., the syntactic and semantic combinatorial possibilities of each item analyzed.
These valence descriptions provide critical information on the mapping between form and meaning; NLP and more broadly, natural language understanding (NLU) require such mapping. 
%is what NLP and Natural Language Understanding (NLU) require.

At the heart of the work is the \textbf{semantic frame}, a script-like knowledge structure that facilitates inference within and across events, situations, relations, etc. 
FrameNet defines a semantic frame in terms of its \textbf{frame elements} (FEs), or participants in the scene that the frame captures; a \textbf{lexical unit} (LU)\label{LU} is a pairing of a lemma and a frame, thus characterizing that LU in terms of the frame that it evokes.
Valence descriptions derive from the annotation of FEs, i.e. \textbf{semantic roles}, on example sentences that illustrate the linguistic manifestation of the participants in a scene for the target of analysis.
%FEs are in fact triples of information; they also provide information about the phrase type (PT) and the grammatical function of the annotated FE. 
%Automatic processes recommend GFs and PTs, which annotators correct, when necessary.
% Example \# \ref{buy}
The first sentence in Figure~\ref{fig:illustration} illustrates annotation with respect to the verb \textit{buy}, which FN defines in terms of the \texttt{Commerce\_buy} frame, whose FEs are a \textsc{{\textcolor{blue}{Buyer}}}, \textsc{{\textcolor{red}{Seller}}}, \textsc{{\textcolor{green}{Goods}}}, and \textsc{{\textcolor{violet}{Money}}}.\footnote{Frame names appear in \texttt{Typewriter} font; FE names are in \textsc{Small Caps}; and LUs are in \textit{italics}.}

% \begin{enumerate}
%     \item \textcolor{blue}{Chuck} \textcolor{blue} {$_{\textsc{Buyer}}$} \textbf{\textcolor{black}{BOUGHT}}
% \textcolor{green}{a car} \textcolor{green}{$_{\textsc{Goods}}$}
% \textcolor{red}{from Jerry} \textcolor{red}{$_{\textsc{Seller}}$} \textcolor{violet}{for \$2,000} \textcolor{violet} {$_{\textsc{Money}}$}\label{buy}
% \end{enumerate}

%%NI: I like your commented sentence better :D

% cf. #3800, Table: Statistics of the dataset from FrameNet
%https://2021.aclweb.org/calls/reproducibility-checklist/

%Ayush to correct numbers based on those for FN 1.7

The FrameNet\footnote{\url{https://framenet.icsi.berkeley.edu/fndrupal/framenet_request_data}} database (version 1.7) holds 1,224 frames, 10,478 frame-specific FEs (in lexical frames),\footnote{FrameNet distinguishes between lexical and non-lexical frames, where the latter do not have associated annotation sets.} over 13,500 LUs.
The primary annotations are in the form of nearly 203,000 manually annotated sentences providing information about the mapping between form and meaning in English; these are called the \textbf{lexicographic} annotations. 
A subset of the sentences with lexicographic annotations contain annotations for all possible frames of meaning in them; FrameNet calls this subset full-text annotations.
Despite FrameNet's costly annotation efforts, 38\% of the over 13,500 LUs in the database remain without annotation. 
That is, a significant amount of LUs in the database have no associated annotated sentences to serve as training data for downstream NLP applications.


\subsection{Frame Semantic Role Labeling}
\label{SRL}
Semantic role labeling (\textbf{SRL)} involves automatically labeling who did what to whom in a text document.
SRL systems facilitate developing {NLP} applications, like question answering
\citep{shenlap07using}, machine translation \citep{pedersen01},
and text summarization \citep{Han16}, to name but a few.
Frame semantic role labeling (\textbf{frame-SRL)} is a special type of SRL where the task is to identify target tokens (which evoke a frame of meaning), the frame itself (of target LUs) and FEs, or semantic roles, in text. 
% A type of linguistic structure prediction \citep{smith2011}, frame-SRL depends on identifying target LUs and their frames \citep{das10probabilistic}, also structure prediction tasks.
%%NI: Frankly I do not really understand this sentence. I wonder if it could be eliminated?
The relationship between frames and their respective FEs requires that the system first identify the correct frame (FrameID) to identify the correct FEs (ArgID).
Identifying the frame incorrectly necessarily means incorrect FE identification.\footnote{\citet{semeval/Baker07} also considered correct identification of the spans of a dependent of a lexical unit, even if the frame and by definition the FEs were identified incorrectly.}
In practice, frame-SRL is usually implemented as a pipeline of structured prediction \cite{smith2011} tasks: identifying targets and LUs, frames, and finally the FEs \cite{das10probabilistic}.

Using an early version of FN data \citep{FNearly}, \citet{Dans02} developed the first SRL system, which also
%Partially motivated by FN's manually annotated data, \citet{Dans02} 
initiated SRL as a now well-recognized task in the field.
Recent years have seen the development of several (relatively) high-performing SRL systems. 
SEMAFOR \citep{das2014frame}
uses a pipeline of discrete, manually designed feature-based linear classifiers for target identification, frame identification (FrameID), and argument identification (ArgID). 
The core constraints of frame-semantic analyses, e.g. not repeating core FEs, are satisfied via
% @swabha: Will you add a sentence that defines "integer linear programming"?
integer linear programming.
PathLSTM \citep{Roth:16} uses neural features to embed path relationships between frames and FEs, in a pipeline similar to that of SEMAFOR.
\citet{yang-mitchell-2017-joint} use a joint model to leverage Propbank SRL annotations to improve frame-SRL.
\sesame \cite{DBLP:journals/corr/SwayamdiptaTDS17,swayamdiptaEtAl18syntactic} uses an unconstrained, neural approach in a pipeline %similar to that of
like SEMAFOR and PathLSTM. 
%(Section \ref{SRL}). 
%%NI: I would eliminate the next sentence--it seems spurious
Continuous representations and a sophisticated global model based on semi-Markov conditional random fields \citep{conf/nips/SarawagiC04} improve identifying arguments.
We employ \sesame\footnote{\url{https://github.com/swabhs/open-sesame}} as the baseline of choice in our experiments (\S\ref{sec:experiments}).
With the exception of a few approaches, like that of \citet{yang-mitchell-2017-joint}, most prior work uses only the full-text annotations for frame-SRL; we present experiments considering the larger set of lexicographic annotations as well.

%Expanding FrameNet is critical for its use in NLP: SRL systems rely on the data and such data are needed for downstream applications.

%\textbf{NI:} You've already said this last bit--I would eliminate it

% \subsubsection{SRL Systems}
% Using a an early version of FrameNet data \citep{FNearly}, \citet{Dans02} developed the first SRL system. FN's manually annotated data motivated (in part) \citet{Dans02}'s development of SRL; and that work also initiated SRL as a now well-recognized task in the field.

%Among those SRL systems, a number are worth mentioning, namely \citet{das2014frame} and \citet{Roth:16}. \citet{das2014frame} built on previous work \citep{das10probabilistic} that...

%With their dependence on FrameNet annotation for training data, 
%the quality and quantity of available manually annotated affects their performance.

% Move this section to after the description of our task?

==> 3-method.tex <==
\section{Method: Data Augmentation with Sister LUs}
\label{sec:methodology}

%\subsection{Hypothesis}
%%NI: DO you really need sub-sections here? I would be inclined to eliminate them.
%%NI: Suggest replacing this subsection with this: 
%The set of LUs associated with a given frame share common semantic properties and can be considered near-synonyms in many instances. This fact has motivated the use of these LU sets for paraphrasing, where one LU from the set replaces another, resulting in an alternative phrasing. For example, \citet{mutaphrase07} produced paraphrases based on the relationship among LUs of a frame or closely related frames, thereby augmenting a meager data set for use in speech recognition. Similarly, LUs common to a given frame tend to follow the same annotation structure: i.e., the arguments of a LU in a frame consist of the same FEs, regardless of the LU.\footnote{Two or more FEs might be part of a \textit{core set}, yet only one will be realized for valid annotation. For a given frame, different LUs may not realize all the same FEs in all examples.} Note the parallel annotation for  \# \ref{buy} shown above and \# \ref{purchase}. On this basis, we hypothesize that existing annotations can inform the automated generation of annotation for \textbf{un}annotated LUs in a given frame.


The relationship among LUs in a frame
motivates examining their use for paraphrasing, where one LU replaces another resulting in an alternative phrasing of a sentence.
%%NI: Maybe a bit more explanation: "The set of LUs associated with a given FN frame necessarily share common semantic properties, and are near-synonyms in many instances. This fact has motivated the use of these LU sets for paraphrasing, where one LU from the set replaces another, yielding an alternative phrasing. For example,
\citet{mutaphrase07} produced paraphrases based on the relationship among LUs of a frame or closely related frames, augmenting a meager data set for use in speech recognition.
%\textbf{add stuff relating to current automatic paraphrasing/machine translation, writing tools} 

Most importantly, LUs in a frame tend overwhelmingly to follow the same annotation structure: the arguments of a lexical unit in a frame consist of the same FEs, regardless of the LU.\footnote{Two or more FEs might be part of a \textit{core set}, yet only one will be realized for valid annotation. For a given frame, different LUs may not realize all the same FEs in all examples.} 
Note the parallel annotation for the two sentences in Figure~\ref{fig:illustration} for the verbs, \textit{buy} and \textit{purchase}.
% \noindent
We use this critical insight in our work, hypothesizing that existing annotation would inform the automated generation of annotation for \textbf{un}annotated LUs in a given frame.

% \begin{enumerate}
%     \setcounter{enumi}{1}
%     \item \textcolor{blue}{Chuck} \textcolor{blue} {$_{\textsc{Buyer}}$} \textbf{\textcolor{black}{PURCHASED}}
% \textcolor{green}{a car} \textcolor{green}{$_{\textsc{Goods}}$ }
% \textcolor{red}{from Jerry} \textcolor{red}{$_{\textsc{Seller}}$} \textcolor{violet}{for \$2,000} \textcolor{violet} {$_{\textsc{Money}}$} \label{purchase}
% \end{enumerate}



%\subsection{Dataset Creation} \label{augmenteddata}
%%NI: rename the section: "Dataset creation"? or something similar?
%%\textbf{NI:} If subsections eliminated, use a transitional phrase like "To this end" to connect the following to the above.
To this end,
\citet{FSautoanno19} defined \textbf{Sister Lexical Unit} as any LU for which annotation exists in a frame, and whose annotation can serve as a model to generate new annotation. A \textbf{Sister} is the LU with annotation and an \textbf{EmptyLU} lacks annotation; the Sister LU and the Empty LU must be of the same part of speech.

%\textbf{NI:} A bit confusing--you define a sister LU as one that has annotation, but then call both annotated and unannotated LUs Sisters.

To generate augmented labeled data, we first identified all EmptyLUs. For each such LU, we identified a corresponding Sister, specifically, the LU with the greatest number of annotation sets and of the same POS as the EmptyLU in a given frame.
%\textbf{NI:} Shouldn't it be "one of its corresponding Sisters", since you are choosing one of a set of possibilities? 
We replaced each occurrence of a Sister in an annotated sentence with the EmptyLU. The replacement process included steps to ensure that the newly generated instance included the correct word forms, i.e., singular and plural forms of nouns or conjugated verbs of a Sister LU, following the strategy that \citet{rastogdurm14} employed, which augmented FN using a paraphrase database \citep{ganitkevitch13ppdb} to add new lemmas and then rewrote existing annotated sentences with those lemmas.

%\textbf{NI:} Replace the rest of the section with: 
%In each of a Sister's  annotated sentences, we replaced its occurrence of Sister with an "EmptyLU". The replacement process included steps to ensure that the newly generated instance included the correct word forms, i.e., singular and plural forms of nouns or conjugated verbs of a Sister  LU, following the strategy that \citet{rastogdurm14} employed, which augmented FN using a paraphrase database \citep{ganitkevitch13ppdb} to add new lemmas.
% The replacement process identified 2,805 previously unannotated LUs in the FrameNet database. 
%Of these, approximately 500 LUs either were multiword expressions (MWEs) or had an MWE as a potential Sister \#1; because the replacement process often yielded  ungrammatical sentences for MWEs, eliminated MWEs from the data, leaving 2,300 previously unannotated LUs.

We transferred each sentence in the annotation set of the Sister into that of each EmptyLU, and replaced instances of the Sister with those of the EmptyLU. 
The replacement process ensured that newly generated data included correct word forms, i.e., singular and plural forms of nouns, conjugated verbs, or those with tense marking. 
%This phase is similar to part of \citet{rastogdurm14}, which augmented FN using a paraphrase database \citep{ganitkevitch13ppdb} to add new lemmas and rewrote existing annotated sentences with those lemmas.
%and gained a threefold increase in coverage at 65\% precision.

%For example, FrameNet has defined the % choose new frame! \texttt{Change\_position\_on\_a\_scale} frame with two core FEs: 

%That frame includes a \textbf{Sister \# 2} LU, \textbf{contract}.v, whose associated Sister \# 1 is \textbf{fall}.v. Example \#\ref{fall} shows the FE annotation of \textbf{Sister \# 1}, where the relevant word form is \textit{falling}. Example \ref{contract} shows an instance of the newly annotated sentence for the target \textbf{contract}.v.

% Colors are great, although I'm not sure that they'll show up in the publication. I think that ACL only uses black/white. Regardless, we need to add the FE names that go with each constituent. I suspect we'll have more than one example, so we should number the examples.

%\begin{enumerate}
%\item \textcolor{green}{Marginal costs} \textcolor{blue}{are} %\textbf{FALLING} \textcolor{pink}{slightly} \textcolor{blue}{, as %illustrated by curve MC, so the industry is a natural monopoly.}
%\end{enumerate} 
% Actually, for a number of reasons (which aren't relevant to the point of the paper, I want to choose another example.

%\begin{enumerate}
%\setcounter{enumi}{2}
%\item \textcolor{blue}{Marginal costs}\textcolor{blue}$_{\textsc{Attribute}}$ \textcolor{black}{are \textbf{FALLING}}
%\textcolor{magenta}{slightly}\textcolor{magenta}$_{\textsc{Manner}}$ as illustrated by....\label{fall}
%\end{enumerate}

Ensuring agreement of tense, person, and number between instances of a sister and an EmptyLU required replacing the original word forms with those of the same grammatical number for nouns and tense, person, and number for verbs. 
However, this does not always yield correct results, e.g., for lemmas with irregular plural or past tense forms, as in \textit{ox, oxen} and \textit{bring, brought}.
% \footnote{Our open-source augmentation code is found at \url{https://github.com/ayush-pancholy/sister-help}.}
%after cleaning it up).
%(Section \ref{analysis} discusses categories of linguistic errors .)

%\begin{enumerate}
%\setcounter{enumi}{3}
%\item \textcolor{blue}{Marginal costs}\textcolor{blue}$_{\textsc{Attribute}}$ \textcolor{black}{are \textbf{CONTRACTING}}
%\textcolor{magenta}{slightly} \textcolor{magenta}$_{\textsc{Manner}}$ as illustrated by....\label{contract}
%\end{enumerate}



%sentences containing words that have irregular endings, replacements may be pluralized or conjugated incorrectly or insufficiently.

%Because of the particular word form of the optimizer target word \textit{falling}, simply replacing it with the base form \textit{contract} would not result in a grammatical sentence. Instead, \textit{contracting} is the appropriate replacement. As such, using several simple rules for inserting the replacement facilitated ensuring that the augmented data also included correct word forms. 

% I'll summarize the rules in short paragraphs so that we can make use of the space that they currently use.
%\begin{enumerate}
%    \item If the optimizer is a noun,
%    \begin{enumerate}
%        \item If the instance ends in 's' and the base form does not, a plural form is inferred. As such, the optimizable lexical unit is adjusted as follows:
%        \begin{enumerate}
%            \item If the base form of the optimizable lexical unit ends in 's,' 'sh,' 'ch,' 'x,' or 'z,' an 'es' suffix is added for pluralization;
%            \item Else, an 's' suffix is added for pluralization.
%        \end{enumerate}
%        \item Else, the base form of the optimizable lexical unit is assumed the correct replacement.
%    \end{enumerate}
%    \item If the optimizer is a verb,
%    \begin{enumerate}
%        \item If the instance of the optimizer ends with 'ing,' the optimizable lexical unit is adjusted by adding 'ing' unless it ends with 'e,' in which case first remove the 'e'.
%        \item If the instance of the optimizer ends with 's, appended an 's' to the optimizable target.
%        \item If the instance of the optimizer ends with 'd,' is appended to the suffix 'ed' to the optimizable target unless it ends with 'e,' in which case only append 'd'.
%        \item Else, the base form of the optimizable lexical unit is assumed to be the correct replacement.
%    \end{enumerate}
%    \item Else, the base form of the optimizable lexical unit is assumed to be the correct replacement.
%\end{enumerate}

\subsection{Candidates for Augmentation}
\label{subsec:augmented_data}

The aforementioned process identified 2,805 previously unannotated LUs, of which approximately 500 either were multiword expressions (MWEs) or had an MWE as a potential Sister. 
Thus, the process added at least one sentence to each previously empty annotation set, yielding the potential to provide new annotation for (approximately)
45\% of the unannotated LUs in FrameNet 1.7.
See Table~\ref{tab:examples} in the Appendix~\ref{sec:app:qualitative} for a few pairs of sister and empty LU pairs.
The replacement process did not always yield grammatically correct results. Sometimes FrameNet (arbitrarily) treats MWEs as single LUs, and using a MWE (as a Sister or an EmptyLU) often resulted in ungrammatical sentences. Thus, we also eliminated MWEs from the data in this work, resulting in 2,300 previously unannotated LUs, eligible for augmentation.
%as in sentences with words that have irregular plurals or verb forms. (See \ref{analysis} for discussion.)




==> 4-experiments.tex <==

\section{Experiments}
\label{sec:experiments}

\input{sections/tables/results}


To test the idea of leveraging frame-specific annotation to generate new annotation for LUs lacking any, we wish to compare the performance of our approach with a baseline model.
This facilitates determining the extent to which our augmentation algorithm would improve SRL performance, and thus (potentially) contribute to the FrameNet corpus.
Our augmentation approach is applied to FrameNet version 1.7.


\subsection{Training Data}
\label{subsec:data}

%%NI: eliminate next paragraph? Seems obvious. Remove "Instead" from next
In principle, our data augmentation algorithm (\S\ref{sec:methodology}) could provide new annotation for 2,300 LUs (\S\ref{subsec:augmented_data}), all of which could be used for training.
However, we wish to determine whether using augmented data improves performance on the existing test sets. %%Doing so requires that our test set contain annotation associated with the augmented data, a state of affairs that cannot occur.
% in the training data that our algorithm produced.
% But, appropriate testing of a frame-SRL model with the resulting data is impossible since previously unannotated LUs would not exist in the testing dataset. 
Additionally, care must be taken to avoid the logical flaw of using augmentation algorithm from producing labeled sentences specifically for the test set: the process would circularly assume that the algorithm offers accurate labelling. 

We addressed this issue by adjusting the training data for the baseline: we removed annotation from 1,500 randomly selected LUs from the lexicographic portion of the training data for FN 1.7.
Each of these 1,500 LUs functions as EmptyLUs when stripped of their annotation. 
Our baseline model was trained with the remaining lexicographic annotations. 
Our full model was trained on data given by the augmentation algorithm to re-annotate the 1,500 LUs, in addition to the data used for the baseline.
% This adjustment allowed us to use the standard FrameNet 1.7 development and test sets, following \citet{DBLP:journals/corr/SwayamdiptaTDS17}.
Note that not all LUs are eligible for training in \sesame, which involves a pre-processing step to remove those LUs incompatible with the parser; Table~\ref{tab: Results} provides the final training data statistics.

In addition to the lexicographic annotations, both the baseline and the augmented setup use all the full-text annotations in FrameNet 1.7.
Our training data adjustments above allow using the standard validation and test sets for FrameNet 1.7, following \citet{DBLP:journals/corr/SwayamdiptaTDS17}.

%Defining processes to include SRL into FrameNet's development constitutes a longer-term goal of this work.\footnote{Much more testing (of numerous factors) than what this report provides is required to evaluate the viability of including SRL into FrameNet's existing primarily manual process.} 
%For example, would active learning improve the results? Is human-in-the-loop SRL faster and as accurate as FrameNet's manual annotation?}

\subsection{Model and Hyperparameters}
\label{subsec:model}

All of our experiments were performed using the non-syntactic model provided in \sesame \citep{DBLP:journals/corr/SwayamdiptaTDS17, swayamdiptaEtAl18syntactic}.
We follow the basic setup in \sesame which assumes gold targets for FrameID and gold frames for ArgID.
We left most hyperparameters associated with \sesame at their default values, but decreased the learning rate for training the ArgID stage to $0.0001$ from its original value of $0.0005$. 
The decrease allowed training ArgID on the entire dataset in three epochs without error, which serves reproducibility requirements.


\subsection{Results}
\label{sec:results}

Table \ref{tab: Results} presents test and validation set performances comparing two \sesame models, trained with and without the augmented data for ArgID and FrameID. 
%% NI: YOU need to explain  FrameID and ArgID -- I can assume what they are, but they should be defined
%Note that 
%We do not report \textbf{P}(recision) or \textbf{R}(ecall) for the devset runs. 
All measures in the experimental setting outperformed the baseline, highlighting the value of data augmentation. 
Although our main interest was testing the system's performance for ArgID (i.e., identifying semantic roles / FEs for given frame-LU annotations) of the augmented data, we also observed improvement in the identification of frames.
%as part of its process.
%\textbf{NI:} This previous sentence is mostly incomprehensible to me. I do not see what the second clause means or how it relates to the first clause. 
% Thus, we also considered if the newly generated augmented data affected the FrameID score.
%% Also, it is still unclear what you are saying about the Frame ID score. Is it that you were looking for the argument ID results, but since \sesame also reports Frame ID you looked at that too? In any case, why were you not concerned about Frame ID to begin with?
The results in the experimental setting show an absolute improvement of 2.7 in F1 on ArgID and 1.6 in F1 on FrameID.\footnote{We further experimented with cross validation settings for both FrameID and ArgID; however, the runtime of \sesame was prohibitively slow in this setting.}


\subsection{Error Analysis and Discussion}
\label{analysis}

%that the augmentation script produced
%\footnote{Unlike other studies that also evaluated correctly identifying the span of text, even if the FE was not correct, this work did evaluate correct spans.}

%%NI: Here you talk about the ungrammatical sentences, which had been discussed above in the generation section. Why isn't this bit included there instead of being presented as part of error analysis? Are you saying that any errors were a result of the ungrammatical sentences? That seems unlikely...and seems to be contradicted by what you say later on about FrameID errors etc. If not, what percentage of errors were due to grammatical  errors?
At times the augmentation algorithm produced ungrammatical sentences. 
We do not believe that errors occurred because of ungrammatical sentences. Still, FrameNet would not conjure producing data with ungrammatical sentences.\footnote{A complete manual analysis of the data remains to be done. In future extensions of this work, we will report such an analysis, including the percentage of grammatical sentences.}
A manual analysis of a random sample of LUs showed three categories of errors: (a) word form mismatch; (b) incorrect or missing marker; and (c) semantic mismatch, examples of which appear in (a) - (c):

\begin{description}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
  \item (a) *The moon was now \textit{occlude} by clouds.\label{wf}
  \item (b) *And he \textit{complained} the endless squeeze on cash.
  \item (c) ?The faint \textit{flash} from a street light showed him the outline of a hedge.\label{sem}
\end{description}

\noindent
The semantic mismatch in (c) holds between \textit{faint}.a and \textit{flash}.n, yielding a semantically odd sentence not an ungrammatical one. 
By definition, a \textit{flash} would not be \textit{faint}.\footnote{The results showed several types of semantic mismatch.
Space limitations preclude discussing all of them here.}

%for example, semantic narrowing, e.g. while \textit{flock}.n and \textit{group}.n are Sister LUs, \textit{flock} cannot replace \textit{group} without changing the meaning of a sentence.

% What's the total number of new annotations? How much augmented data did our algorithm produce? I think that number is important, especially since I want to compare it with the Brazilian results (increase of 13%). 
%I think that our method may have increased the number of annotated LUs by 20\%, and does not rely on f2f relations to infer labels across related frames (as Brazilians did, while relying on an incorrect understanding of FEs with the same name in different frames).

% 2795/5130 = 54% ACK!!: only 2300/5130 because of MWEs = 45%
% Total LUs 13,572 of which 5130 have no annotation.
% 2795 + 8404 = 11,199/13,572 = 82.5%
% 61.9 - 59.3 = 2.6 : F1 - baseline

% 2.6/59.3 = 4.38%


% What measure would show if the results are statistically significant?


%\begin{itemize}
%\itemsep-0.25em
%    \item augmentation issues; snippets of data
%    \item linguistic analysis: categories of error types
%    \item why did the F1 score increase only by the amount that it did?
    %ref. Swabha's github re: performance w/lexicographic annotation); check Swabs' github pg Test Section 2
    % Since OS uses word forms rather than lemmas, then incorrect word form could affect F1 score.
%\end{itemize}    

%\textbf{NI:} Here you start to provide some of the explanation of FrameID and ArgID that needs to come much earlier. 
%The relationship between frames and their FEs requires that the system first identify the correct frame (FrameID) to identify the right FEs (ArgID). %of a sentence. Identifying the frame incorrectly necessarily means incorrect FE identification.
%%NI: So, what percentage of the ArgID errors resulted from FrameID errors?
%FrameNet has defined FEs frame-specifically; when the system chooses the wrong frame, it will err on FEs.
%\footnote{FEs may appear the same in different frames only because FrameNet uses a shorthand to identify FEs.} 
Recall that incorrectly identifying a frame necessarily yields incorrect FEs (ArgID). The analysis showed that errors occurred with highly polysemous lemmas, such as \textit{make}.v, where FrameNet has 10 LUs; in (d), \sesame misidentified 
\textit{making}.v as \texttt{Manufacturing}, not \texttt{Earnings\_and\_losses}. Similarly, (e) is a misidentification of \textit{gathering} as \texttt{Food\_gathering}, not \texttt{Come\_together}. Note the metaphorical use of the verb in (e), compared to literal senses of the lemma \textit{gather}.v. %included in FrameNet.

\begin{description}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
  \item (d) I like working and \textit{making} money.
  \item (e) ...the debate on welfare reform is \textit{gathering} like a storm at sea...
\end{description}

% % @swabha:
% \subsection{Cross-Validation Experiment}\label{eval}
% % Evaluating the results for statistical significance would be ideal. 
% To increase confidence in the experiment's results, we are doing 5-fold cross-validation (CV) on the system's performance with the augmented data.\footnote{Limited access to sufficient computing power given pandemic-related issues delayed running these tests. Results will be available before the final submission deadline.} For this test, we compiled two data sets: Set A includes the annotated sentences from the original FrameNet 1.7 lexicographic data; Set B includes the sentences that the augmentation algorithm generated. We divided Set A into five subsets. For each iteration, we used one subset of Set A as the devset, adding the other four to Set B to produce a training set. 
% %Table \ref{CV} 
% We will report the dev F1 scores of each iteration's model for both ArgID and FrameID.

%\textbf{NI:} I may be ignorant here, but I've never seen anyone provide results for each fold of a cross-fold validation, but rather, one usually reports the mean of the model skill scores along with a measure of the variance of the skill scores (e.g. standard deviation or standard error).

%\begin{table}[h]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%CV Run & 1 & 2 & 3 & 4 & 5 \\ \hline
%ArgID & 00.0  & 00.0  & 00.0  & 00.0 & 00.0  \\ \hline
%FrameID & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\ \hline
%\end{tabular}
%\caption{Cross-Validation Dev F1 Scores}\label{CV}
%\end{table}

% Populate Table 2 after CV runs complete. Discuss these F1 scores relative to those in Table 1 to emphasize significance (if so). 

% Comparison to similar work:
    % compare with SOA SRL paper that doesn't do this!
    % Pavlick et al 2015.
    % Brazilian paper


% Add something about ability of code to incorporate GF \& PT information.


==> 5-related.tex <==
\section{Related Work}
\label{sec:related}



Data augmentation in the context of FrameNet and SRL is not novel. \citet{pavlick15FN} created an expanded FN via automatic paraphrasing and crowdsourcing to confirm frame assignment of LUs.
%\citet{hartmanngenerat16} used linked lexical resources to generate role labeled training data, producing classifiers trained on the generated data equaling that of a standard supervised setting. 
\citet{hartmannassess17} used automatically generated training data
by linking FrameNet, PropBank, and VerbNet to study the differences among those resources in frame assignment and
semantic role classification. The results showed that the augmented data performed as well as the training data for these tasks on German texts.
With similar goals to those of this work, \citet{AugmentFN20} proposed augmenting FN annotation using notions of lexical, syntactic, or semantic equivalence, and FN's frame-to-frame relations (Inheritance, Using, SubFrame, etc.) to \textit{infer} annotations across related frames, producing a 13\% increase in annotation. 
%(See Section \ref{eval} for a comparison.)



==> 6-future.tex <==

\section{Conclusion and Future Work}
\label{sec:future}

We outlined an approach to Frame-SRL that seeks to leverage existing annotation in a frame to generate new annotation for previously unannotated LUs in the same frame, by exploiting the already identified target and frame of a given lemma.
Further, we demonstrated that augmentation of data improves Frame-SRL performance substantially.
% compare with SOA SRL paper that doesn't do this!
% This work differs from previous studies that employ open-SESAME and would benefit from comparison with such work. 
While we show the advantages of this approach on the open-SESAME baseline, future work might involve studying if using this type of data augmentation will yield improvements on a state-of-the-art SRL system, e.g. \citet{FeiEtAl21}.

Several other interesting directions for future work exist, including the following: refining the augmentation algorithm to produce more grammatical sentences; streamlining open-SESAME's code to run more efficiently; use active-learning to inform the data generation and to assist in the SRL task; and experimentation with other computational techniques, as suggested by \citet{FSautoanno19}.
These plans will advance defining processes to include Frame-SRL into FrameNet's development process, the ultimate goal of this work.\footnote{Rigorous testing of multiple factors will be required to evaluate the viability of including Frame-SRL into FrameNet's existing primarily manual process.} 



==> tables/results.tex <==
% \resizebox{\textwidth}{!}{
\begin{table*}[ht]
\small
%NOTE: As of 5/5/2021, this table should have correct values!
\centering
%\resizebox{\textwidth}{%}

%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
% & \multicolumn{1}{c|}{ArgID (dev)} & \multicolumn{1}{c|}{FrameID (dev)} & % \multicolumn{3}{c|}{ArgID (test)} & \multicolumn{3}{c|}{FrameID (test)} \\ %\hline
% & F1 & F1 & P & R & F1 & P & R & F1 \\ \hline
%B-OS & 59.3 & 84.7 & 61.8 & 56.9 & 59.2 & 81.1 & 81.1 & 81.1 \\ \hline
%E & 61.9 & 85.3 & 63.6 & 60.3 & 61.9 & 82.7 & 82.7 & 82.7 \\ \hline
%\end{tabular}
\begin{tabular}{lrrrrrrrrr}
\toprule
 & & & \multicolumn{2}{c}{Dev} & \multicolumn{4}{c}{Test}\\
 \cmidrule(lr){4-5}\cmidrule(lr){6-9}
 & \multicolumn{2}{c}{Training Data} & \multicolumn{1}{c}{ArgID} & \multicolumn{1}{c}{FrameID} &   \multicolumn{3}{c}{ArgID} & \multicolumn{1}{c}{FrameID} \\ 
 \cmidrule(lr){2-3} \cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-8}\cmidrule(lr){9-9}
& \#LUs  & \#Lexicographic Annotations & F1 & F1 & P & R & F1 & F1 \\ \midrule
\multirow{2}{*}{\sesame} & 6905 & 164372 & 59.3 & 84.7 & 61.8 & 56.9 & 59.2 & 81.1 \\ 
& 7944 & 260292 & \textbf{61.9} & \textbf{85.3} & \textbf{63.6} & \textbf{60.3} & \textbf{61.9} & \textbf{82.7} \\
\bottomrule
\end{tabular}
\caption{Results comparing the \sesame models trained on the original FrameNet 1.7 data for frame identification (FrameID) and argument identification (ArgID) tasks, with \sesame models trained on our augmented data. 
Data augmentation improves performance on both tasks across all metrics; boldface indicates best performance.
Note that under both settings we consider full-text annotations, a subset of the lexicographic annotations.
Gold-standard frames were used for ArgID, and gold-standard targets for FrameID, in both the baseline and our models.
Development set results only include F1 scores; (by default) \sesame just reports that score.}
\label{tab: Results}
\end{table*} 

% }
